Towards Real-Time Panoptic Narrative Grounding by an End-to-End Grounding Network

Panoptic Narrative Grounding (PNG) is an emerging cross-modal grounding task, which locates the target regions of an image corresponding to the text description. Existing approaches for PNG are mainly based on a two-stage paradigm, which is computationally expensive. In this paper, we propose a one-stage network for real-time PNG, termed End-to-End Panoptic Narrative Grounding network (EPNG), which directly generates masks for referents. Specifically, we propose two innovative designs, i.e., Locality-Perceptive Attention (LPA) and a bidirectional Semantic Alignment Loss (SAL), to properly handle the many-to-many relationship between textual expressions and visual objects. LPA embeds the local spatial priors into attention modeling, i.e., a pixel may belong to multiple masks at different scales, thereby improving segmentation. To help understand the complex semantic relationships, SAL proposes a bidirectional contrastive objective to regularize the semantic consistency inter modalities. Extensive experiments on the PNG benchmark dataset demonstrate the effectiveness and efficiency of our method. Compared to the single-stage baseline, our method achieves a significant improvement of up to 9.4% accuracy. More importantly, our EPNG is 10 times faster than the two-stage model. Meanwhile, the generalization ability of EPNG is also validated by zero-shot experiments on other grounding tasks.

==> tables/table1.tex <==

\begin{table*}[t!]
\centering
\resizebox{1.00\textwidth}{!}{
\begin{tabular}{l|ccccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{|c|}{Average Recall} & \multicolumn{3}{c}{Inference Time} & \multicolumn{3}{|c}{Params} & \multicolumn{3}{|c}{Training Data}\\

\cline{2-15}
 & All & Thing & Stuff & Single & Plural & Stage-1 & Stage-2 & All & Stage-1 & Stage-2 & All & Stage-1 & Stage-2 & All\\
 \hline
 PNG & 55.4 & 56.2 & 54.3 & 56.2 & 48.8 & 100ms & 7ms & 107ms & 21.0M & 240.3M & 261.3M & 1.3M & 0.8M & 2.1M\\

 \hline
 Baseline(ours) & 40.3 & 34.5 &  50.5 & 42.3 & 31.4 & - & - & \textbf{9.5ms} & \multirow{3}{*}{-} & \multirow{3}{*}{-} & \multirow{3}{*}{\textbf{76.5M}} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{\textbf{0.8M}}\\
 EPNG(ours) & 49.7 & 45.6 & 55.5 & 50.2 & 45.1 & -& -& 11ms& & & & & & \\
 EPNG$^\ast$ & \textbf{58.3} & \textbf{54.6} & \textbf{63.0} & \textbf{59.3} & \textbf{47.9} & - & - & 11ms & & & & - & - & 2.1M\\
 \bottomrule
\end{tabular}}
%}
\caption{Comparison of the EPNG and the previous two-stage method. Baseline means the same design with EPNG except for LPA and SAL.
%add
EPNG$^\ast$ is trained with the same data as PNG.}
\label{table1}
\end{table*}

==> tables/table2.tex <==
% tabel2
\begin{table*}[t]
\centering

\begin{tabular}{c|c|ccc|ccc|ccc|c}
\toprule
 \multirow{2}{*}{Model}& \multirow{2}{*}{Type} & \multicolumn{3}{|c|}{Time} & \multicolumn{3}{|c|}{Params} & \multicolumn{3}{|c|}{Training Data} & \multirow{2}{*}{Training}\\

\cline{3-11}
 &  & Stage-1 & Stage-2 & All & Stage-1 & Stage-2 & All & Stage-1 & Stage-2 & All & \\
 \hline
 PNG & serial & 100ms & 48ms & 146ms & 21.0M & 240.3M & 261.3M & 1.3M & 0.8M & 2.1M & offline \\
 % \multirow{2}{*}{PNG} & serial & 100ms & 48ms & 146ms & \multirow{2}{*}{21.0M} & \multirow{2}{*}{240.3M} & \multirow{2}{*}{261.3M} & \multirow{2}{*}{1.3M} & \multirow{2}{*}{0.8M} & \multirow{2}{*}{2.1M} & \multirow{2}{*}{offline} \\

 \hline
 \multirow{2}{*}{EEPG} & serial & - & - & \textbf{72ms} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{\textbf{76.5M}} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{0.8M} & \multirow{2}{*}{online} \\
\cline{2-5}
  & parallel & - & - & \textbf{11ms} &  &  &  &  &  &  &  \\
 \bottomrule
\end{tabular}
%}
\caption{Commands that must not be used}
\label{table2}
\end{table*}

==> tables/table3.tex <==
% tabel3
\begin{table}[t]
\centering

%\resizebox{1.00\columnwidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
\multirow{2}{*}{Communicator} & \multicolumn{5}{c}{Average Recall} \\

\cline{2-6}
 & All & Thing & Stuff & Single & Plural\\
 \hline
 %- & 45.3 & 42.1 & 52.2 & 46.9 & 41.5 \\
 %\hline
 w/o PE & 42.8 & 36.5 & 52.1 & 44.2 & 32.5\\
 %\hline
 PE & 46.7 & 43.0 & 52.9 & 47.6 & 42.4\\
 SPE & 46.1 & 41.8 & 52.2 & 46.6 & 42.2\\
 DPE & 45.9 & 41.5 & 52.0 & 46.5 & 40.3\\
 RPE & 45.3 & 42.1 & 52.2 & 46.9 & 41.5 \\
 %\hline
 LPA & \textbf{49.7} & \textbf{45.6} & \textbf{55.5} & \textbf{50.2} & \textbf{45.1} \\
 \bottomrule
\end{tabular}
%}
\caption{Ablation study of the LPA module, where %``-'' denotes no communicator, 
``w/o PE'' denotes an LPA module that does not use any distance or location information, and ``PE'' means use position embedding \cite{vaswani2017attention} instead of the distance embedding in LPA.}
\label{table2}
\end{table} 

==> tables/table4.tex <==
% tabel4
\begin{table}[t]
\centering
\resizebox{1.00\columnwidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
\multirow{2}{*}{Loss} & \multicolumn{5}{c}{Average Recall} \\

\cline{2-6}
 & All & Thing & Stuff & Single & Plural\\
 %\hline
 %BCE & 42.4 & 36.9 & 50.3 & 44.4 & 33.4 \\
 \hline
 BCE + Dice & 43.7 & 38.5 & 49.6 & 43.7 & 37.6\\
 %BCE + SAL & 45.5 & 41.8 & 53.0 & 47.1 & 40.9\\
 %\hline
 BCE + Dice + SAL & \textbf{49.7} & \textbf{45.6} & \textbf{55.5} & \textbf{50.2} & \textbf{45.1} \\
 \bottomrule
\end{tabular}}
%}
\caption{Ablation study of the SAL. %For all the settings, we ensure that all the encoders are LPA.
}
\label{table3}
\end{table}

==> tables/table5.tex <==
% tabel5
\begin{table}[t]
\centering
\resizebox{1.00\columnwidth}{!}{
\begin{tabular}{c|c|c|cccc}
\toprule
 \multicolumn{2}{c|}{Dataset} & Type & mIoU & p@0.3 & p@0.4 & p@0.5\\
 \hline
 \multirow{4}{*}{RefCOCO} & \multirow{2}{*}{testA} & rand & 9.1 & 2.5 & 0.8 & 0.1 \\
 \cline{3-3}
  & & zs & 61.4 & 42.5 & 26.5 & 12.4\\
  \cline{2-7}
  & \multirow{2}{*}{testB} & rand & 10.9 & 3.3 & 1.3 & 0.3 \\
 \cline{3-3}
  & & zs & 35.1 & 22.4 & 13.4 & 7.8\\
  
  \hline
 \multirow{4}{*}{RefCOCO+} & \multirow{2}{*}{testA} & rand & 9.3 & 2.6 & 0.7 & 0.2 \\
 \cline{3-3}
  & & zs & 60.8 & 41.1 & 25.6 & 11.9\\
  \cline{2-7}
  & \multirow{2}{*}{testB} & rand & 11.9 & 3.8 & 1.4 & 0.3 \\
 \cline{3-3}
  & & zs & 41.4 & 27.4 & 16.3 & 9.4\\
  
\hline
 \multirow{2}{*}{RefCOCOg} & \multirow{2}{*}{test} & rand & 12.1 & 4.0 & 1.5 & 0.6 \\
 \cline{3-3}
  & & zs  & 55.1 & 40.1 & 27.3 & 16.3\\

 \bottomrule
\end{tabular}}
%}
\caption{zs results of EPNG on RES. EPNG is not trained with RES data.  We average the IoU of every case as the mIoU.}
\label{table4}
\end{table}
